Evolution of entanglement under an Ising-like Hamiltonian with particle losses

We present analytical compact solution for the density matrix and correlation functions of two collective-macroscopic spins evolving via Ising-like Hamiltonian in the presence of particle losses. The losses introduce non-local phase noise which destroys highly entangled states arising in the evolution. On the other hand, the states appearing at relatively short timescales, possessing EPR-like entanglement will survive. Applying our solutions to the recently proposed scheme to entangle two Bose-Einstein condensates, we estimate the optimal number of atoms for EPR correlations.

==> commands.tex <==
% !TeX root = triplewell.tex


%%%%%%%%%%%%%%%%%%%

\newcommand{\gpe}{Gross-Pitaevskii equation\xspace}
\newcommand{\bec}{Bose-Einstein condensate\xspace}
\newcommand{\becs}{Bose-Einstein condensates\xspace}

\newcommand{\ray}{Rayleigh\xspace}


\newcommand{\qu}[1]{``#1''}


\newcommand{\figref}[1]{FIG.~\ref{#1}}

%%%%%%%%%%%%%%%%%% math abbreviations %%%%%%%%%%%%%%%%%%
\newcommand{\bb}[1]{\left(#1\right)}                                		% (..)
\newcommand{\absv}[1]{\left|#1\right|}                             			% |..|
\newcommand{\absvsq}[1]{\absv{#1}^2}	                            		% |..|^2
\newcommand{\comm}[2]{\left[#1, #2\right]}									% [.., ..]
\newcommand{\bra}[1]{\left\langle#1\right|}  								% <...|
\newcommand{\ket}[1]{\left|#1\right\rangle}  							 	% |...>
\newcommand{\braket}[2]{\left\langle#1\middle|#2\right\rangle}  			% <...|...>
\newcommand{\braketop}[3]{\left\langle#1\middle|#2\middle|#3\right\rangle}	% <...|...|...>
\newcommand{\meanv}[1]{\left\langle#1\right\rangle}							% <...>
\newcommand{\hastobe}{\stackrel{!}{=}}                              		% !=
\newcommand{\unit}[1]{\ensuremath{\, \mathrm{#1}}}                     		% unit




\renewcommand{\vec}[1]{\boldsymbol{#1}}                             % vector

\newcommand{\partiald}[1]{\frac{\partial}{\partial #1}}             % d/(d..)
\newcommand{\timed}{\frac{{\rm d}}{{\rm d} t}}             % d/(d..)
\newcommand{\laplace}{\operatorname{\nabla^2}}                        % laplace

\newcommand{\integralb}[3]{\int\limits_{#1}^{#2} \! \mathrm{d} #3\,} 	% integral
\newcommand{\integral}[1]{\int \! \mathrm{d} #1\,}                    % integral without limits
\newcommand{\integralf}[2]{\int \! \frac{\mathrm{d} #1}{#2}\,}        % integral with a fraction (e.g. int dk/sqrt(2pi))
\newcommand{\intvol}{\integral{^3r}}								% integral over the whole space
\newcommand{\intvolp}{\integral{^3r'}}								% integral over the whole space d^3r'
\newcommand{\intvold}{\intvol\!\intvolp}								% double integral over the whole space d^3r d^3r'

\newcommand{\fourier}[1]{\mathcal{F}\!\left\{#1\right\}}
\newcommand{\invfourier}[1]{\mathcal{F}^{-1}\!\left\{#1\right\}}


\newcommand{\deltaf}{\ensuremath{\operatorname{\delta}}\xspace}	    % delta function
\newcommand{\expf}[1]{\ensuremath{\exp\bb{#1}}\xspace}	    		% exp(...)
\newcommand{\ef}[1]{\ensuremath{\operatorname{e}^{#1}}\xspace}	    % e^(...)


% physical abbreviations

\newcommand{\hamil}{\ensuremath{\operatorname{{\hat{H}}}}\xspace} % Hamilton operator
\newcommand{\heff}{\ensuremath{\operatorname{{\hat{H}_\text{eff}}}}\xspace} % effective Hamilton operator
\newcommand{\heffn}{\ensuremath{\operatorname{{H_\text{eff}}}}\xspace} % effective Hamilton, number


\newcommand{\aop}{\ensuremath{\hat{a}}\xspace} % annihilation operator
\newcommand{\aopd}{\ensuremath{\hat{a}^\dagger}\xspace} % creation operator
\newcommand{\nop}{\ensuremath{\hat{n}}\xspace} % number operator


\newcommand{\Na}{\ensuremath{{N_\text{A}}}\xspace}                               % N_A

\newcommand{\I}{\dot{\imath}}

\newcommand{\Dx}{\Delta x}
\newcommand{\Dy}{\Delta y}
\newcommand{\Dz}{\Delta z}
\newcommand{\Dt}{\Delta t}

\newcommand{\hc}{\hat{c}}
\newcommand{\hcd}{\hat{c}^{\dagger}}
\newcommand{\na}{\hat{n}_{0}}
\newcommand{\nb}{\hat{n}_{1}}
\newcommand{\nc}{\hat{n}_{c}}
%\newcommand{\hef}{\hat{H}_{\text{eff}}}


\newcommand{\wc}{\omega_c}
\newcommand{\wa}{\omega_a}
\newcommand{\wl}{\omega_L}


\newcommand{\vece}{\ket{\epsilon_1, \epsilon_2, \ldots, \epsilon_N}}
\newcommand{\epi}[1]{\epsilon_{#1}}

\newcommand{\ketp}[1]{\ket{#1}_{\rm PH}}
\newcommand{\keta}[1]{\ket{#1}_{\rm AT}}
\newcommand{\brap}[1]{\bra{#1}_{\rm PH}}
\newcommand{\braa}[1]{\bra{#1}_{\rm AT}}

% Spin physics

\newcommand{\sx}{\sigma^x}
\newcommand{\sxi}[1]{\sigma^x_{#1}}
\newcommand{\sy}{\sigma^y}
\newcommand{\syi}[1]{\sigma^y_{#1}}
\newcommand{\sz}{\sigma^z}
\newcommand{\szi}[1]{\sigma^z_{#1}}

\newcommand{\sM}{\sigma^{-}}
\newcommand{\sMi}[1]{\sigma^{-}_{#1}}
\newcommand{\sP}{\sigma^{+}}
\newcommand{\sPi}[1]{\sigma^{+}_{#1}}

\newcommand*{\upk}{\ensuremath{\ket{\uparrow}}}
\newcommand*{\upb}{\ensuremath{\bra{\uparrow}}}

\newcommand*{\stbk}{\ensuremath{\ket{b}}}
\newcommand*{\stak}{\ensuremath{\ket{a}}}
\newcommand*{\stbb}{\ensuremath{\bra{b}}}
\newcommand*{\stab}{\ensuremath{\bra{a}}}

\newcommand*{\proj}[1]{\ket{#1}\bra{#1}}
\newcommand*{\proji}[1]{\ket{#1}\bra{#1}_i}

\newcommand*{\opb}{\ensuremath{b}}
\newcommand*{\opa}{\ensuremath{a}}
\newcommand*{\opbd}{\ensuremath{b^{\dagger}}}
\newcommand*{\opad}{\ensuremath{a^{\dagger}}}


\newcommand*{\cFD}{\ensuremath{c^{\dagger}}}
\newcommand*{\cF}{\ensuremath{c}}

\newcommand*{\downk}{\ensuremath{\ket{\downarrow}}}
\newcommand*{\downb}{\ensuremath{\bra{\downarrow}}}

\newcommand*{\Sx}{\ensuremath{\hat{S}_x}}
\newcommand*{\Sy}{\ensuremath{\hat{S}_y}}
\newcommand*{\Sz}{\ensuremath{\hat{S}_z}}
\newcommand*{\Splus}{\ensuremath{\hat{S}_+}}
\newcommand*{\Sminus}{\ensuremath{\hat{S}_-}}
\newcommand*{\Sperp}{\ensuremath{\hat{S}_\perp}}



\newcommand{\adj}[1]{\ensuremath{#1^\dagger}}

\newcommand*{\cdag}{\ensuremath{\adj{c}}}



\newcommand*{\exck}{\ensuremath{\ket{e}}}
\newcommand*{\excb}{\ensuremath{\bra{e}}}
\newcommand*{\oat}{\ensuremath{\omega_a}}

% Decoherence

\newcommand{\gambar}{\bar{\Gamma}}
\newcommand{\gamrm}{\gambar_{\rm Ram}\xspace}
\newcommand{\gamry}{\gambar_{\rm Ray}\xspace}



